Image2SSM: Reimagining Statistical Shape Models from Images with Radial Basis Functions

Statistical shape modeling (SSM) is an essential tool for analyzing variations in anatomical morphology. In a typical SSM pipeline, 3D anatomical images, gone through segmentation and rigid registration, are represented using lower-dimensional shape features, on which statistical analysis can be performed. Various methods for constructing compact shape representations have been proposed, but they involve laborious and costly steps. We propose Image2SSM, a novel deep-learning-based approach for SSM that leverages image-segmentation pairs to learn a radial-basis-function (RBF)-based representation of shapes directly from images. This RBF-based shape representation offers a rich self-supervised signal for the network to estimate a continuous, yet compact representation of the underlying surface that can adapt to complex geometries in a data-driven manner. Image2SSM can characterize populations of biological structures of interest by constructing statistical landmark-based shape models of ensembles of anatomical shapes while requiring minimal parameter tuning and no user assistance. Once trained, Image2SSM can be used to infer low-dimensional shape representations from new unsegmented images, paving the way toward scalable approaches for SSM, especially when dealing with large cohorts. Experiments on synthetic and real datasets show the efficacy of the proposed method compared to the state-of-art correspondence-based method for SSM.

==> resources.tex <==
\section{Resources}
This section will include equations, calculations, and network architecture diagrams. For reference only, will be removed in final.

\subsection{RBF Solving and Querying Basics}
\ssmmodel\ is a network (see Fig. \ref{arch}) that takes in a 3D image $I$ and outputs an RBF TPS surface respresentation. It trains using corresponding pairs of images $I$ and distance transforms $D_{dt}$ which come from the same population/distribution. The resulting surface is defined by a set of $m$ particles \P, a set of $m$ normals $\N$, and a column vector $\w = \{w_1, w_2, ..., w_{3m}, c_0, c_1, c_2, c_3\}$. This representation can be converted to other surface representations (mesh, SDF, etc.) \cite{Turk1999VariationalIS, rbf_surface1}. The network itself $\ssmmodel m(I)$ only outputs a set of $m$ particles \P\ and a set of $m$ normals $\N$. 

\w\ is computed by solving an RBF system of equations on the zero-crossing and the dipoles of the surface, that is, we evaluate to 0 at the surface, $s \in \mathbb{R}$ at $s$ units from the surface in the positive normal direction and $-s$ at $s$ units from the surface in the negative normal direction. This allows us to have a well-defined surface in 3 dimensions. Thus we build the vector of zero crossing and dipoles

\begin{equation}
\begin{split}
    \P^+ = \{\p_1, ..., \p_m, \p_1 + s\n/|\n|, ... , \p_m + s\n/|\n|,  \p_1 - s\n/|\n|, ... , \p_m - s\n/|\n| \}
\end{split}
\end{equation}

Before discussing how to solve for \w, we will show that we can evaluate distances to the surface at any coordinate $(x, y, z)$ using the method detailed in \cite{Turk1999VariationalIS, rbf_surface1}, with which we can evaluate a distance transform or mesh. Suppose we want to evaluate the values at coordinates $\X = \{\x_1, \x_2, ... , \x_k\}$, we can use the function:

\begin{equation}
\begin{split}
    d(\x_i) = \sum_{j=1}^{3m} w_j \phi(x_i, p^+_j) + c_0 + \x_1^x c_1 + \x_1^y c_2 + \x_1^z c_3,
\end{split}
\end{equation}

where $\phi$ is the chosen RBF function, which can vary, but is usually the biharmonic radial basis function $\phi(\x,\y) =(|\x-\y|_2)^2\log(|\x-\y|_2)$. All $\x$ of interest can be evaluated at once using a matrix multiplication

\begin{equation}
\begin{split}
    g_{\P^+, \w}(\X) = \A_{\P^+}(\X)\w=\bf d,
\end{split}
\end{equation}

which in expanded matrix form becomes,

\begin{equation}
\begin{split}
    \A(\X) =
    \begin{bmatrix} 
        \phi(\x_1, p^+_1) & \phi(\x_1, p^+_2) & \dots  & \phi(\x_1, p^+_{3m}) & 1 & \x_1^x & \x_1^y & \x_1^z &\\
        \phi(\x_2, p^+_1) & \phi(\x_2, p^+_2) & \dots  & \phi(\x_2, p^+_{3m}) & 1 & \x_2^x & \x_2^y & \x_2^z &\\
        \vdots & \vdots & & \vdots & \vdots & \vdots & \vdots & \vdots\\
        \phi(\x_k, p^+_1) & \phi(\x_k, p^+_2) & \dots  & \phi(\x_k, p^+_{3m}) & 1 & \x_k^x & \x_k^y & \x_k^z &\\
        1 & 1 & \dots & 1 & 0 & 0 & 0 & 0 & \\
        \x_1^x & \x_2^x & \dots & \x_k^x & 0 & 0 & 0 & 0 & \\
        \x_1^y & \x_2^y & \dots & \x_k^y & 0 & 0 & 0 & 0 & \\
        \x_1^z & \x_2^z & \dots & \x_k^z & 0 & 0 & 0 & 0 & \\
    \end{bmatrix}
\end{split}
\end{equation}

and

\begin{equation}
\begin{split}
    \bf d =
    \begin{bmatrix} 
        d_1 & \\
        d_2 & \\
        \vdots & \\
        d_{k} & \\
        0 & \\
        0 & \\
        0 & \\
        0 & \\
    \end{bmatrix}
\end{split}
\end{equation}

where $d_i$s represent the distances to the surface for each $x_i$.

Given our system, we can then solve for $\w$ using the methods in  \cite{Turk1999VariationalIS, rbf_surface1} by simply using a solve function for $\w$ in

\begin{equation}
\begin{split}
    \A_{\P^+}(\P^+)\w=\bf d,
\end{split}
\end{equation}

with $\bf d$ being 0 for the first $m$ values, $s$ for the next $m$, $-s$ for the following $m$, and four zeroes

\begin{equation}
\begin{split}
    \bf d =
    \begin{bmatrix} 
        0 & \\
        \vdots & \\
        0 & \\
        s & \\
        \vdots & \\
        s & \\
        -s & \\
        \vdots & \\
        -s & \\
        0 & \\
        0 & \\
        0 & \\
        0 & \\
    \end{bmatrix}.
\end{split}
\end{equation}

All in all, having $\P, \N$, and $\w$ or the equivalent $\P^+$ and $\w$ are sufficient to represent a surface in 3D by using dipoles to impose surface information. 

\subsection{NovaSSM Loss Functions}
As it currently stands, the loss function of \ssmmodel\ can be divided in 3 parts (shown in figure \ref{losses}), written as follows:

\begin{equation}
\begin{split}
  L(I, D_{dt}, D_{xyz}, nb, d_{nb}) &= L_{Surface} (I, D_{dt}, D_{xyz}) + \\
  & L_{Sampling} (I, D_{dt}, nb, d_{nb}) + \\
  & L_{Correspondence} (I).
\end{split}
\end{equation}

The objective is hence to minimize $L$ over $\P$ and $\N$

\begin{equation}
\begin{split}
  \min_{\P, \N} L(I, D_{dt}, D_{xyz}, nb, d_{nb})
\end{split}
\end{equation}

Each of these can be implemented in different proposed ways explained below, which are currently being tested. In this section, let's assume that we have solved the system and have the values of $\P^+$, $\A_{\P^+}$ and $\w$ handy, so we are able to compute $g_{\P^+, \w}(\X)$ at will.

\subsubsection{Surface Loss} The surface loss concerns how close particles are to the true surface and how close the normals are to the true surface normals at any coordinate of interest. For this, we minimize the distance metric 

\begin{equation}
\begin{split}
  L_{Surface} (I, D_{dt}, D_{xyz}) = \sum_{i}^m d_1(g_{\P^+, \w}(\p_i), D_{dt}(\p_i)) + d_2(n_i, D_{xyz}(\p_i))
\end{split}
\end{equation}

where $D_{dt}(\x)$ is the value of the distance transform at coordinate $\x$, $D_{xyz}(\x)$ is the gradient with respect to $x, y$ and $z$ components of the distance transform at coordinate $\x$, $d_1$ is a distance metric for distance to the surface (MSE or L1), and $d_2$ is a distance metric for the normal ($1-CosSim()$ and MSE work well). 
Thus far, we have mainly been trying different metrics for $d_1$ and $d_2$ but are open to other approaches.

\subsubsection{Sampling Loss} The sampling objective aims to dictate the distribution of particles on the shapes in order to enable statistical shape modeling. 

We have so far formulated two different approaches, condition number (CN) and narrow band (NB). 

The \textbf{condition number approach} uses the RBF matrix's condition number $\kappa(\A) = 	\lVert \A \rVert_F \lVert \A^{-1} \rVert_F$. The condition number is (very roughly) the rate at which the solution $\w$ will change with respect to a change in $\bf d$. When the condition number is minimized, it will tend to spread particles out evenly because if two particles are too close together, they will conflict with each other, changing multiple $\w$s rapidly if $\bf d$ changes at all. This should be further studied, as I can't claim to fully understand this approach. The condition number (CN) loss can be written

\begin{equation}
\begin{split}
  L_{Sampling(CN)} (I) = \lVert \A_{\P^+}(\P^+) \rVert_F \lVert \A_{\P^+}(\P^+) \rVert_F
\end{split}
\end{equation}

The \textbf{narrow band approach} extracts the values at the narrow band of the distance transform, a narrow region close to the surface where we are interested in computing the area to the surface accurately (other areas can be inferred or not that important). These narrow band points $nb$ and their corresponding values $d_{nb}$ are extracted as a preprocessing step to speed up iterations. The goal of this loss is to spread particles in a way that we not only evaluate the control points correctly but also the interpolated surface points around the control points correctly as well. We hence use all points that are close of which interpolated values we are interested in to enforce to attempt to achieve this. Thus far, this approach has had mixed success. It can be written as

\begin{equation}
\begin{split}
  L_{Sampling(NB)} (I, nb, d_{nb}) = \sum_{i}^{nb} d_3(g_{\P^+, \w}(nb_i), d_{nb, i})
\end{split}
\end{equation}

where $nb_i$ is a point within the narrow band, $d_{nb, i}$ is the evaluation value at the point $nb_i$, and $d_3$ is a distance metric (we use MSE, but can be L1).

\subsection{Architecture Diagrams}
This is where we include architectural diagrams.

\begin{figure}
\includegraphics[width=\textwidth]{figures/network}
\caption{This is the current architecture we are running. This is, of course, subject to change.} \label{arch}
\end{figure}

\begin{figure}
\includegraphics[width=\textwidth]{figures/losses}
\caption{This is how the losses are currently being applied to the output of the network..} \label{losses}
\end{figure}

\subsection{References}
This is a collection of all references we have gathered.

\subsubsection{Original RBF surface representation papers} 
1. Reconstruction and Representation of 3D Objects with Radial Basis
Functions. \cite{rbf_surface1} 

2. Variational Implicit Surfaces. \cite{Turk1999VariationalIS}

\subsubsection{ShapeWorks papers}
1. Leveraging Unsupervised Image Registration for Discovery of Landmark Shape Descriptor \cite{BHALODIA2021102157}

2. Shapeworks: particle-based shape correspondence and visualization software \cite{cates2017shapeworks}

\subsubsection{Sent by Shireen on 01/15}
1. Deep Implicit Templates for 3D Shape Representation. \cite{DBLP:journals/corr/abs-2011-14565}

2. PaMIR: Parametric Model-Conditioned Implicit Representation for Image-Based Human Reconstruction. \cite{9321139}

3. SAL: Sign Agnostic Learning of Shapes from Raw Data. \cite{DBLP:journals/corr/abs-1911-10414}
4. Deep Implicit Moving Least-Squares Functions for 3D Reconstruction. \cite{Liu_2021_CVPR}

5. DeepSDF: Learning Continuous Signed Distance Functions for Shape Representation. \cite{Park_2019_CVPR}

6. Sign-Agnostic Implicit Learning of Surface Self-Similarities for Shape Modeling and Reconstruction From Raw Point Clouds. \cite{Zhao_2021_CVPR}

7. Surface Reconstruction from Point Clouds: A
Survey and a Benchmark\cite{Huang_2022}

